External leg corrections in the unitarity method

Unitarity cuts diverge in the channel of a single massive external fermion. We propose an off-shell continuation of the momentum that allows a finite evaluation of the unitarity cuts. If the cut is taken with complete amplitudes on each side, our continuation and expansion around the on-shell configuration produces the finite contribution to the bubble coefficient. Finite parts in the expansion of the external leg counterterms must be included explicitly as well.

==> DIAGRAMS/HBBloopMOMon.tex <==
\unitlength=0.35bp%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(6.5,10.)(0.,){/ScalarDash}{0}
\FALabel(3.25,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(13.,14.)(0.,){/Straight}{-1}
\FALabel(16.2808,15.5544)[b]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(13.,6.)(0.,){/Straight}{1}
\FALabel(16.2808,4.44558)[t]{\scriptsize $b(k_3,c_3)$}
\FAProp(6.5,10.)(13.,14.)(0.,){/Straight}{1}
%\FALabel(9.20801,13.1807)[br]{\scriptsize $b$}
\FAProp(6.5,10.)(13.,6.)(0.,){/Straight}{-1}
%\FALabel(9.20801,6.81927)[tr]{\scriptsize $b$}
\FAProp(13.,14.)(13.,6.)(0.,){/Cycles}{0}
%\FALabel(14.974,10.)[l]{\scriptsize $g$}
\FAVert(6.5,10.){0}
\FAVert(13.,14.){0}
\FAVert(13.,6.){0}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(17.3,6.5)(0.,){/Straight}{1}
%\FALabel(18.9227,6.62494)[bl]{\scriptsize $b$}
\FAProp(11.,10.)(13.7,8.5)(0.,){/Straight}{-1}
%\FALabel(12.0773,8.37506)[tr]{\scriptsize $b$}
\FAProp(17.3,6.5)(13.7,8.5)(-0.8,){/Straight}{1}
\FALabel(14.4273,5.18506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(17.3,6.5)(13.7,8.5)(0.8,){/Cycles}{0}
%\FALabel(16.5727,9.81494)[bl]{\scriptsize $g$}
\FAVert(11.,10.){0}
\FAVert(17.3,6.5){0}
\FAVert(13.7,8.5){0}
\FALabel(10.,-1.)[b]{$\mathcal{M}_{H\to b \bar b}(k_1,k_2,k_3)$}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(17.3,13.5)(0.,){/Straight}{-1}
%\FALabel(18.3773,15.1249)[br]{\scriptsize $b$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(11.,10.)(13.7,11.5)(0.,){/Straight}{1}
%\FALabel(12.0773,11.6249)[br]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(-0.8,){/Straight}{-1}
%\FALabel(16.5727,10.1851)[tl]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(0.8,){/Cycles}{0}
\FALabel(14.4273,14.8149)[br]{\scriptsize $b(k_2,c_2)$}
\FAVert(11.,10.){0}
\FAVert(17.3,13.5){0}
\FAVert(13.7,11.5){0}
\end{feynartspicture}



==> DIAGRAMS/HBBtree.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{$H$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{$b$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{$b$}
\FAVert(11.,10.){0}
\end{feynartspicture}



==> DIAGRAMS/HBBtreeC.tex <==
\unitlength=0.42bp%
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
\FAProp(18.,16.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
\FAProp(18.,4.)(9.,10.)(0.,){/Straight}{1}
\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(9.3,9.8)(18.,9.8)(0.,){/Cycles}{0}
\FALabel(15.,8.4)[dl]{\scriptsize $g(k_4,A_4)$}
\FAVert(9.,10.){-1}
\FALabel(9.,10.)[]{\scriptsize $T$}
\FALabel(10.,0.)[b]{$\mathcal{M}_{H\to b g \bar b}(k_1,k_2,k_4,k_3)$}
\end{feynartspicture}
%
%
\hspace{0.1cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(9.,10.)(0.,){/Cycles}{0}
\FALabel(4.22725,11.6251)[tr]{\scriptsize $g (k_1,A_1)$}
\FAProp(0.,5.)(9.,10.)(0.,){/Straight}{1}
\FALabel(4.77275,6.62506)[tl]{\scriptsize $b (k_2, c_2)$}
\FAProp(20.,10.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(14.5,11.07)[b]{\scriptsize $b (k_3, c_3)$}
\FAVert(9.,10.){0}
\FALabel(10.,0.)[b]{$\mathcal{M}_{g b \to b}(k_1,k_2,k_3)$}
\end{feynartspicture}
%
%
\hspace{0.1cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(9.,10.)(0.,){/Cycles}{0}
\FALabel(4.22725,11.6251)[tr]{\scriptsize $g (k_1,A_1)$}
\FAProp(0.,5.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(4.77275,6.62506)[tl]{\scriptsize $b (k_2, c_2)$}
\FAProp(20.,10.)(9.,10.)(0.,){/Straight}{+1}
\FALabel(14.5,11.07)[b]{\scriptsize $b (k_3, c_3)$}
\FAVert(9.,10.){0}
\FALabel(10.,0.)[b]{$\mathcal{M}_{g \bar b \to \bar b}(k_1,k_2,k_3)$}
\end{feynartspicture}


==> DIAGRAMS/HBBtreeS.tex <==
\unitlength=0.35bp%
%
%
\hspace{3cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(9.,10.)(0.,){/ScalarDash}{0}
\FAProp(0.,6.)(9.,10.)(0.,){/Straight}{1}
\FALabel(0.,12.8)[t]{\scriptsize $H (k_1)$}
\FALabel(0.,7.2)[tr]{\scriptsize $b (k_2,c)$}
\FAProp(18.,16.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(14,14)[br]{\scriptsize $b (k_3, c_3)$}
\FAProp(18.,4.)(9.,10.)(0.,){/Straight}{1}
\FALabel(14.,6.)[tr]{\scriptsize $b(k_5,c_5)$}
\FAProp(9.,10.)(18.,10.)(0.,){/Straight}{1}
\FALabel(15.,8.5)[dl]{\scriptsize $b(k_4,c)$}
\FAVert(9.,10.){-1}
\FALabel(9.,10.)[]{\scriptsize $T$}
\FALabel(10.,-1.)[b]{$\mathcal{M}_{H b\to b b \bar b}(k_1,\ell,k_3,\ell,k_5)$}
\end{feynartspicture}
%
%
\hspace{3cm}
% 
%


==> DIAGRAMS/loop.tex <==
\unitlength=0.3bp%
%
%
% LOOP UNCUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}
%
%
\hspace{0.5cm}  % LOOP DOUBLE CUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\myblue
\FAProp(13.75,15.)(13.75,5.)(0.,){/ScalarDash}{0}
\black
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}
%
%
\hspace{0.5cm}  % LOOP SINGLE CUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\myblue
\FAProp(13.75,10.5)(13.75,5.)(0.,){/ScalarDash}{0}
\black
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}


==> DIAGRAMS/treeL.tex <==
\unitlength=0.22bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
%
\FAProp(11.,10.)(16.,14.)(0.,){/Cycles}{0}
\FALabel(19.3,13.2)[t]{\tiny $g (\ell, A)$}
\FAProp(11.,10.)(16., 6.)(0.,){/Straight}{1}
\FALabel(22.,6.8)[b]{\tiny $t (K-\ell, c')$}
%
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAVert(6.5,10.){-1}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}



==> DIAGRAMS/treeR.tex <==
\unitlength=0.22bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(7.5,10.)(0.,){/Cycles}{0}
\FALabel(3.37021,11.6903)[tr]{\tiny $g (\ell, A)$}
\FAProp(0.,6.)(7.5,10.)(0.,){/Straight}{1}
\FALabel(4.12979,6.69032)[tl]{\tiny $t (K-\ell, c')$}
\FAProp(7.5,10.)(15.,10.)(0.,){/Straight}{1}
\FALabel(13.25,11.07)[b]{\tiny $t (K,c)$}
\FAVert(7.5,10.){0}
\end{feynartspicture}



==> DIAGRAMS/ttggCT_copy.tex <==
%\unitlength=0.42bp%
\unitlength=0.25bp
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\scriptsize
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$2$}
\FAProp(0.,5.)(3.,7.5)(0.,){/Straight}{-1}
\FALabel(2.01229,5.53926)[tl]{$1$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$3$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$4$}
\FAProp(3.,7.5)(6.,10.)(0.,){/Straight}{-1}
%\FALabel(5.01229,8.03926)[tl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,11.77)[b]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,7.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$2$}
\FAProp(0.,5.)(5.,5.5)(0.,){/Straight}{-1}
\FALabel(2.65423,4.18769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(5.,5.5)(10.,6.)(0.,){/Straight}{-1}
%\FALabel(7.65423,4.68769)[t]{$t$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
%\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(5.,5.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(3.,12.5)(0.,){/Straight}{1}
\FALabel(0.987714,13.0393)[tr]{$2$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$1$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$3$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$4$}
\FAProp(3.,12.5)(6.,10.)(0.,){/Straight}{1}
%\FALabel(5.01229,11.9607)[bl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,8.93)[t]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,12.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.,14.5)(0.,){/Straight}{1}
\FALabel(2.65423,15.8123)[b]{$2$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(5.,14.5)(10.,14.)(0.,){/Straight}{1}
%\FALabel(7.65423,15.3123)[b]{$t$}
\FAProp(10.,6.)(10.,14.)(0.,){/Straight}{-1}
%\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,6.){0}
\FAVert(10.,14.){0}
\FAVert(5.,14.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$2$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{-1}
%\FALabel(11.07,12.)[l]{$t$}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{1}
%\FALabel(8.93,8.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){2}
\end{feynartspicture}



==> DIAGRAMS/ttggCTdef.tex <==
\unitlength=0.42bp%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$t$}
\FAProp(0.,5.)(3.,7.5)(0.,){/Straight}{-1}
\FALabel(2.01229,5.53926)[tl]{$t$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$g$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$g$}
\FAProp(3.,7.5)(6.,10.)(0.,){/Straight}{-1}
\FALabel(5.01229,8.03926)[tl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(10.,11.77)[b]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,7.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$t$}
\FAProp(0.,5.)(5.,5.5)(0.,){/Straight}{-1}
\FALabel(2.65423,4.18769)[t]{$t$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$g$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$g$}
\FAProp(5.,5.5)(10.,6.)(0.,){/Straight}{-1}
\FALabel(7.65423,4.68769)[t]{$t$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(5.,5.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$t$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$t$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$g$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$g$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{-1}
\FALabel(11.07,12.)[l]{$t$}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{1}
\FALabel(8.93,8.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){2}
\end{feynartspicture}


